Articulate That Object Part (ATOP): 3D Part Articulation via Text and Motion Personalization

We present ATOP (Articulate That Object Part), a novel few-shot method based on motion personalization to articulate a static 3D object with respect to a part and its motion as prescribed in a text prompt. Given the scarcity of available datasets with motion attribute annotations, existing methods struggle to generalize well in this task. In our work, the text input allows us to tap into the power of modern-day diffusion models to generate plausible motion samples for the right object category and part. In turn, the input 3D object provides ``image prompting'' to personalize the generated motion to the very input object. Our method starts with a few-shot finetuning to inject articulation awareness to current diffusion models to learn a unique motion identifier associated with the target object part. Our finetuning is applied to a pre-trained diffusion model for controllable multi-view motion generation, trained with a small collection of reference motion frames demonstrating appropriate part motion. The resulting motion model can then be employed to realize plausible motion of the input 3D object from multiple views. At last, we transfer the personalized motion to the 3D space of the object via differentiable rendering to optimize part articulation parameters by a score distillation sampling loss. Experiments on PartNet-Mobility and ACD datasets demonstrate that our method can generate realistic motion samples with higher accuracy, leading to more generalizable 3D motion predictions compared to prior approaches in the few-shot setting.

==> remove/1_introduction_old.tex <==
%\vspace{-7mm}
\section{Introduction}
\label{sec:intro}

Everyday objects in the 3D world we live in undergo various movements and articulations. 
%How the different parts of a 3D object move and interact with each other reflects the object's intended functions. As such, 
The ability to model and reason about object articulations in 3D plays an important role in simulation, design, autonomous systems, as well as robotic vision and manipulation.
%
Over the past ten years, there has been a steady build-up of digital 3D assets, from ShapeNet~\cite{chang2015shapenet} (3M models)  in the early days, to efforts on improving the assets' structure (e.g., PartNet~\cite{mo2019partnet} with 27K finely segmented models) and quality (e.g., Amazon Berkeley Objects (ABO)~\cite{collins2022abo} with $\sim$8K models), and to the latest and largest open-source repository Objaverse-XL~\cite{deitke2023objaversexluniverse10m3d} (10M+ models).
However, very few, if any, of these models come with part motions. Predominantly, they were all constructed in their rest (i.e., unarticulated) states. To our knowledge, the largest 3D datasets with part articulations, PartNet-Mobility~\cite{xiang2020sapien} and 
Shape2Motion~\cite{wang2019shape2motion}, only contain 2,346 and 2,440 {\em manually\/} annotated synthetic models, respectively. Clearly, human annotations are expensive in terms of time, cost, and expertise --- they are not scalable to endow large volumes of 3D assets with articulations. 

In this paper, we wish to develop a learning method to generate {\em plausible\/} and {\em accurate\/} articulations for {\em any\/} given 3D object, {\em without\/} relying on any human-annotated 3D part motions as most existing methods~\cite{hu2017learning,wang2019shape2motion,abbatematteo2019learning,mo2021where2act,jain2021screwnet,yan2020rpm,jiang2022opd} do. In addition, we would also like to solve this problem in a {\em few-shot\/} setting, making the task even more challenging. %Earlier approaches~\cite{wang2019shape2motion, yan2020rpm, jiang2022opd} infer the motion parameters in a feed-forward manner, with training on datasets with human annotations. 
With the recent success of {\em video diffusion models\/}~\cite{blattmann2023stable,wang2024vc,xing2024dynamicrafter,guo2023animatediff, wan2025wan, yang2024cogvideox, li2024puppet}, it is natural to leverage their zero-shot and open vocabulary capabilities to first generate motion samples for our target object. \nt{These motion samples can then be fed to a generalized multi-view video generator like SV4D \cite{xie2024sv4d, yao2025sv4d} to generate motion from multiple views. These motion samples can then be used to perform \nt{multi-view}-to-3D motion transfer. This approach is (3D) annotation-free, hence more scalable, but faces \nt{four} key challenges to obtain accurate 3D part articulations:


\begin{itemize}[leftmargin=*]


\item First, while SOTA video diffusion models 
can attain unprecedented visual quality for open-domain text-to-video generation, they are not yet well trained or sufficiently adaptive to generating articulations of \nt{variety} of everyday objects (e.g., even something as simple as a folding chair), especially when typical {\em piecewise rigidity\/} is expected. For e.g. Fig. \ref{fig:diff_articulation} (left) shows the video generated from an input image with a text prompt using a state-of-the-art Image-to-Video (I2V) model WAN2.1 \cite{wan2025wan}. 

\item Second, 
%to ensure an \rz{accurate} motion transfer from video to 3D, the motioned object in the generated video must be as close to the target 3D object as possible. 
while current Text-to-Video (T2V) models or \nt{Image-to-Video (I2V) models can generate plausible motions for {\em some \/} referenced object in text or image, to our knowledge, none of the them can ensure that the content in the generated motion is consistent across all the frames with the referenced object.}

\item
\nt{Second, relying only on text prompts makes it difficult to control the movement of individual parts, which is essential for accurate articulation estimation. As can be seen in Fig. ~\ref{fig:diff_articulation} (left) current diffusion models struggle to provide precise control over the motion of {\em specific \/} parts. A more suitable model for this task could be the one with a more explicit control in the form of for e.g. ``drags" \cite{li2024puppet}. However, these models does not always guarantee to give correct and plausible video output. As can be seen in Fig. ~\ref{fig:diff_articulation} }

\item
\nt{Third, even if an accurate monocular video output of part articulation is obtained from an off-the-shelf I2V model, lifting the motion from a single view to multiple views is equally challenging and important so that the articulation from the videos can be faithfully transferred from 2D to 3D space.}

\end{itemize}


\input{figures/diff_articulation}




% Recently, there has been a surge of attempts to train foundational generative models \nt{to learn a motion prior for part-level dynamics \cite{li2024dragapart, li2024puppet}. However, in order to train such models large amount of annotation efforts are required (for e.g. annotating drags) which again, is expensive in-terms of time, cost and expertise.} %In addition, the scarcity of annotated datasets significantly limits their generalization ability.
% %over few  is mainly restricted to categories for which ample data samples is available for e.g. Storage and Tables. Not only that the methods which rely on training foundational generative model require explicit control in which direction the part should move in the form of drags making the annotation process for large scale training even more costly. 
% %
% With the recent success of {\em video diffusion models\/}~\cite{blattmann2023stable,wang2024vc,xing2024dynamicrafter,guo2023animatediff, wan2025wan, yang2024cogvideox, li2024puppet}, it is natural to leverage their zero-shot and open vocabulary capabilities to first generate motion samples for our target object, \nt{then use a multi-view video generator like SV4D \cite{xie2024sv4d, yao2025sv4d} to generate motion sample from multiple views} and then perform a \nt{multi-view}-to-3D motion transfer. This approach is (3D) annotation-free, hence more scalable, but faces \nt{four} key challenges to obtain accurate 3D part articulations:



% %Still, it seems natural to leverage the zero-shot and open vocabulary capabilities of the emerging {\em video diffusion models\/}~\cite{blattmann2023stable,wang2024vc,xing2024dynamicrafter,guo2023animatediff} for motion attribute prediction. By developing our approach on such a foundational model, will help to predict correct part dyanamics which otherwise is not always possible with GPT based approach. However, there are three key challenges to obtain accurate 3D part articulations:


% % to first generate motion videos \av{from multiple views for our target object} and then perform a 2D-to-3D motion transfer. 

% \begin{itemize}[leftmargin=*]
% \item First, while SOTA video diffusion models 
% can attain unprecedented visual quality for open-domain text-to-video generation, they are not yet well trained or sufficiently adaptive to generating articulations of \nt{variety} of everyday objects (e.g., even something as simple as a laptop), especially when typical {\em piecewise rigidity\/} is expected; see Fig. \ref{fig:diff_articulation}. 
% % \sn{I think this is not true particularly with the latest video diffusion models being good enough to do articulations, but one new angle that can be brought about is generating multi-view videos from a image cannot be solved by a single model, for that you need to do i) single image to video ii) video to multi-view video generation, here it is a 2-stage model where there is a chance of error propagation from (i) to (ii) which may affect results. But for our case it is a single stage pipeline.}
% \if 0 
% >>> not so important to have to say in the intro <<<
% One way to remedy this is by reducing the domain gap using large-scale training data such as \cite{li2024puppet}. 
% However, compared to image and video datasets, the availability of such large-scale 4D data is still rather limited.
% \fi
% %
% \item Second, 
% %to ensure an \rz{accurate} motion transfer from video to 3D, the motioned object in the generated video must be as close to the target 3D object as possible. 
% while current text-to-video (T2V) models or \nt{image-to-video (I2V) models can generate plausible motions for {\em some \/} referenced object in text or image, to our knowledge, none of the them can ensure that the content in the generated motion is consistent across all the frames with the referenced object.}

% % can generate plausible motions for {\em some\/} referenced object, to our knowledge, none of them can ensure that the generated motion is exactly of a {\em specific\/} (the target) {\em 3D object\/}}.
% % \sn{This point is the same concern as point 1, issues related to video diffusion models have been solved recently}
% %given cabinet. Hence, the source video generated for the motion transfer must be {\em personalized\/} to the target object.}

% \item
% \nt{Third, current diffusion models struggle to provide precise control over the motion of specific parts. Relying only on text prompts makes it difficult to control the movement of individual parts, which is essential for accurate articulation estimation.}
% %which is crucial for estimating motion attributes of \em each part of the object.

% \item
% \nt{Fourth, even though we obtain an accurate monocular video output of part articulation, generating that motion from multiple views is equally challenging and important so that the articulation from the videos can be faithfully transfered from 2D to 3D space.}
% %which is crucial for estimating motion attributes of \em each part of the object.
% \end{itemize}

% \input{figures/diff_articulation}
% % \input{figures/t2i_articulation}

% \nt{A straightforward solution to this problem would be a zero-shot approach where off-the-shelf models for each of the task (I2V + V2MV) can be leveraged independently. For e.g. given an image of a target 3D object, one can use Puppetmaster \cite{li2024puppet} to generate plausible part motion by giving drag as a prompt as shown in Fig. ~\ref{fig:diff_articulation} (right). The generated video from Puppetmaster can then be fed to another generalized off-the-shelf multi-view generator like SV4D \cite{xie2024sv4d,  yao2025sv4d} to get multi-view part motion samples for the target 3D object. This approach has the potential to scale. However, it suffers from several limitations. First, despite being generalizable, currently, these models are trained with``drag" based ground truth which is manually annotated, hence restricting the scale at which these models can be trained (16k animation samples) compared to standard I2V models which only use text prompt. Second, these methods suffer from ambiguity in the drag signal to clearly identify the correct moving part especially in multi-part scenario. Third, even if I2V model generates a plausible motion, there are chances that multi-view motion generator like SV4D can introduce multi-view inconsistencies in the final motion samples. Because of error propogation in each stage of this two stage pipeline, generating plausible output samples from such a pipeline is challenging as can be seen in Fig. ~\ref{fig:diff_articulation} (right). We conduct two experiments where in the first we try to generate an articulation motion from a latest I2V model like WAN 2.1 \cite{wan2025wan} using a text prompt and an image as shown in this figure (left). The generated video from the I2V model is then fed into SV4D \cite{xie2024sv4d, yao2025sv4d} to generate multi-view motion videos. As it is difficult to control the motion purely using text prompt I2V model fails to generate plausible articulation motion which propagates the error into the multi-view video generator. Similarly, we also experiment with another I2V model PuppetMaster \cite{li2024puppet} which takes a ``drag" as a prompt. As can be seen in the figure (right) because of drag ambiguity in specifying the exact direction of motion, it tries to lift the seat of the chair rather than folding the seat of the chair. This error is than propogated to SV4D which generates implausible videos for estimating the final articulation.


% % \begin{itemize}[leftmargin=*]
% % \item Despite being generalizable, currently, these models are trained with ``drag" based ground truth which is manually annotated, hence restricting the scale at which these models can be trained. For e.g. Puppetmaster \cite{li2024puppet} is trained on only $16k$ animation samples hence limiting its generalization ability compared to image or video diffusion models.
% % \item asadsdf
% % \end{itemize}
% } 

% \nt{Inspired from \cite{ruiz_dreambooth_2023} and to address the above challenges, we present a novel method based on {\em motion personalization \/} to articulate a 3D object in the form of a mesh, using the guidance from a controllable part-aware multi-view motion generator. We propose a single stage light weight model design such that when trained with some reference samples of part motion, the model can then directly hallucinate the motion pattern for a part of a target shape from multiple views using text prompt and multi-view images rendered from the target mesh; see Fig. ~\ref{fig:teaser}}. Our method is coined ATOP, for Articulate That Object Part, and it consists of two steps:
% % \sn{I think we need to change some writing here, as the methodology section is slightly planned to be altered.}
% \begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=2pt, leftmargin=*]
% \nt{\item {\em Finetuning for plausible part motion generation.} This is the key first step to compensate for the lack of articulation awareness by current diffusion models. We finetune a pre-trained multi-view \textit{image} generator, ImageDream~\cite{wang2023imagedream}, for \textit{controllable multi-view motion} generation, using {\em few-shot\/} motion samples available during training. For this, we start from the pre-trained weights of ImageDream and inflate them for video processing, with motion region-of-interest and multi-view controls enabled through text and camera pose conditioning. Once finetuned, given a new target 3D mesh, we render multi-view images and masks of the part which is to be articulated is fed to the diffusion model which \em{hallucinates \/} the {\em desired part motion} from multiple-views, personalized to the target object.}

% % \item {\em Finetuning for category-specific motion video generation.} This is a key first step to compensate for the lack of articulation awareness by current video diffusion models. We finetune a pre-trained multi-view \textit{image} generator, ImageDream~\cite{wang2023imagedream}, for \textit{controllable multi-view video} generation, using {\em few-shot\/} video samples obtained for the target object category, that are of different objects from the target. We start from the pre-trained weights of ImageDream and inflate them for video processing, with motion region-of-interest and multi-view controls enabled through text and camera pose conditioning.

% % \nt{A straight-forward solution to this problem would be to fine-tune an I2V video model like \cite{xing2024dynamicrafter, wan2025wan, guo2023animatediff}}

% % To address these challenges, we present a novel method based on {\em motion personalization\/} to articulate a 3D object in the form of a mesh, with respect to a part prescribed in a {\em text prompt\/}; see Fig.~\ref{fig:teaser}.
% % which can be either user-specified or predicted by existing motion segmentation methods~\cite{jiang2022opd,wang2024active}. 
% % Specifically, the text input allows us to tap into the power of modern-day diffusion models to generate plausible motion samples for the right object category and part. The input 3D object provides {\em image prompting\/} to personalize the generated video to {\em that\/} very object we wish to articulate. 



% % We start from the pre-trained weights of ImageDream and inflate them for multi-view video processing. We opt to expand an image diffusion model for video generation due to its relatively higher articulation awareness, as demonstrated in Fig. \ref{fig:t2i_articulation}. In addition, the signal for controlling part motion (i.e., the specific part we aim to articulate) is established using mask conditioning derived from a segmented mesh.
% % with motion ROI (region-of-interest) and multi-view controls enabled through text and camera pose conditioning.
% % \item {\em Motion video personalization.}
% % We render multi-view images and masks of the part which is to be articulated, for the target 3D mesh. These images, rendered masks, camera poses, and text prompt embeddings are fed to our diffusion model, which \textit{hallucinates} the {\em desired part motion} from multi-views, personalized to the target object.
% \item {\em Multi-view motion-to-mesh motion transfer.}
% Using the personalized output from above, we transfer the plausible video motion to the target 3D object via differentiable rendering, which optimizes the motion axis parameters associated with the prescribed part by a score distillation sample (SDS) loss \cite{poole2022dreamfusion}; see Fig.~\ref{fig:pipeline} for an overview.
% \end{enumerate}

% To our knowledge, ATOP presents the first annotation-free learning framework for generating accurate part articulations of existing 3D objects from text prompts. We present both qualitative and quantitative experiments to show that our method is not only capable of generating realistic personalized motion videos on unseen shapes, but also transferring the motion to 3D meshes, resulting in more accurate articulations in 3D than prior works in a few-shot setting.


% \if 0 

% we first resort to {\em few-shot fine-tuning\/} of a 3D-aware multi-view 
% video diffusion model, namely, ImageDream~\cite{wang2023imagedream}, to generate class-specific motion videos. 
% Our fine-tuning is based on TuneAVideo~\cite{wu2023tune} for multi-view personalized video generation. 
% We start from pre-trained weights of ImageDream models and inflate it to multi-view generation. As a result from this
% first step, if the target object is a laptop, then we are able to generate motion videos showing laptops undergoing
% various articulations, e.g., opening or closing, from text prompts.
% %
% Next, we perform video personalization so as to generate a motion video specifically of the input 3D object, at least
% something as close to it as possible.

% Recently there have been methods proposed, which show one shot or few shot tuning of image diffusion models for Text2Video generation \cite{wu2023tune, qi2023fatezero, wu2023lamp}. These methods have shown the ability to quickly learn a motion pattern from few-shot examples which can then be leveraged for text-based video editing. We propose to use such a finetuning framework for our task of motion video personalization. More precisely we leverage multiview image generation models \cite{wang2023imagedream, shi2023mvdream, long2024wonder3d} as our base to incorporate multiview awareness in the video generation by inflating the pre-trained weights for video processing. In addition to this, we incorporate temporal awareness within the personalized model by adding temporal self-attention layers which are trained using few shot examples provided during training.

% \av{[Note: Should write about video diffusion models, how they are not aware of articulation. Also write about how this method can be used to manipulate the video output which traditional nerf based method cannot. Traditional nerf based 4D reconstruction method cannot be controlled.]}

% \av{[Note: Should write about how it is difficult to articulate just using text description and hence personalization approach. More Controllability!]}

% \fi

% \if 0
% The Amazon Berkeley Objects (ABO)~\cite{collins2022abo} is a recently published, large-scale ($\sim$8K models) dataset of high-quality, artist-created 3D models of 63 categories of real products being sold. While the ABO objects are all associated with product metadata and realistic geometries and material, the 3D models have all been constructed in their ``rest", i.e., unarticulated, poses without revealing their functions. The same is true for the vast majority of 3D models in well-established repositories such as ShapeNet~\cite{chang2015shapenet} (3M models) and PartNet~\cite{mo2019partnet} (27K models with fine-grained segmentation).

% The largest 3D datasets with part articulations, SAPIEN~\cite{xiang2020sapien} and Shape2Motion~\cite{wang2019shape2motion}, only contain 2,346 and 2,440 {\em manually\/} annotated synthetic models, covering 46 and 36 object classes, respectively. Currently, creating articulated 3D models relies on human effort which can be expensive in terms of time, cost and expertise.
% \fi




==> remove/5_results.tex <==
\section{Experiments}
\label{experiments}

\input{figures/qual_mv_results_comparison}


In this section, we present the qualitative and quantitative results of our method's ability to infer 3D motion parameters given only a static segmented mesh as input. Along with it we also compare our multi-view video outputs with other baselines.
\subsection{Dataset and Metrics Details}
We evaluate our approach using the PartNet-Mobility dataset \cite{xiang2020sapien}, following the train-test split of \cite{kim2024partstad, liu2023partslip}. This split contains $8$ shapes for training and the remaining for testing for each category of PartNet-Mobility dataset. Each training shape is rendered into four view videos, capturing articulations like a folding chair’s seat movement. Views are set at azimuth angles of $[45\degree, 135\degree, 225\degree, 315\degree]$, with elevation at $10\degree$ for some categories and $30\degree$ for rest. These views are fixed throughout our experiments. We select the views based on how closely the selected views match the training distribution of camera poses of ImageDream. Each view consists of $10$ frames at $256\times256$ resolution, along with the first frame's binary mask of the part that is to be articulated. To evaluate the generalization ability of our method, we assess its performance not only on the test split of the PartNet Sapien dataset \cite{liu2023partslip, kim2024partstad}, but also conduct {\em zero-shot\/} experiments on $135$ objects from the ACD dataset \cite{iliash2024s2o}, curated by \cite{liu2024singapo}. The ACD dataset features challenging objects sourced from ABO \cite{collins2022abo}, 3D-Future \cite{fu20213d}, and HSSD \cite{khanna2024habitat}. Unlike PartNet-Sapien, which has a lot of structural repetitions, ACD consists of objects that are structurally distinct from each other~\cite{iliash2024s2o}. ACD provides textured segmented meshes with part annotations. We render multi-view images and segmentation masks using the same camera viewpoints used during finetuning. 

\av{We assess our approach in two steps: 1) Multi-View Motion Generation and 2) 3D Motion Axis Parameter estimation. For temporal coherence, we use Frechet Video Distance (\texttt{FVD}) \cite{unterthiner2019fvd}, while text alignment is measured with the \texttt{CLIP} score \cite{CLIP1}. Spatial and temporal consistency are evaluated using \texttt{PSNR} and \texttt{LPIPS} \cite{zhang2018perceptual}. To assess 3D motion axis parameter estimation, we follow \cite{wang2019shape2motion, jiang2022opd} and compute Mean Angular Error (\texttt{MAE}) and Mean Position Error (\texttt{MPE}) of the joint axis. \texttt{MAE} is the dot product between predicted and ground truth motion axes, while \texttt{MPE} is the euclidean distance between their joint origins.}
\subsection{Baselines}
% To the best of our knowledge, this is the first work to address the challenge of 3D mesh articulation via few-shot motion personalization. Consequently, no existing baseline directly takes the same input and produces the same output as ours. Instead, we evaluate individual components of our pipeline by comparing them against suitable baselines for each step. For the multi-view video evaluation step, our model takes a input image with a part mask as input and generates multi-view videos for the part. For this step, we adapt PuppetMaster \cite{li2024puppet} and ImageDream \cite{wang2023imagedream} as our baselines. PuppetMaster \cite{li2024puppet} is an open-vocabulary articulation method that generates a motion articulated video from a input image and a sparse set of motion trajectories (i.e., drags) as user input. Since there is no drag based input to our model, we use the ground-truth part trajectory from the training data to estimate the drags. Imagedream \cite{wang2023imagedream} is a multi-view generation model which generates multi-view images given a single image as input. For the 3D motion transfer step, our pipeline takes a static segmented 3D mesh as input and estimates the 3D motion axis parameters based on the motion output from the multi-view diffusion model. To evaluate this step, we compare with Shape2Motion \cite{wang2019shape2motion} (S2M) and Openable Part Detection \cite{jiang2022opd} (OPD). S2M takes 3D object point cloud as input and estimates the motion parameters, whereas OPD takes a image of the object as input and estimates the motion parameters. We evaluate both the steps of our method along with the baselines on PartNet-Mobility dataset.  
Given the modules used in our approach, we assess the individual components of our pipeline by benchmarking them against appropriate baselines tailored to each step. 
\input{figures/sv4dbaseline_comp}

\subsubsection{Multi-View Motion Generation Baselines.} 
Since no prior work directly predicts {\em multi-view motion} from {\em static multi-view images \/} in a {\em controllable manner\/}, we create a {\em zero-shot\/} baselines where we first use an off-the-shelf state-of-the-art I2V diffusion model to generate video from a static image and then provide the output video to another off-the-shelf state-of-the-art multi-view motion generator to generate multi-view videos. For this baselines we propose two configurations with varying levels of motion control in I2V generation step. In the first configuration, we combine the latest I2V diffusion model WAN $2.1$ \cite{wan2025wan} with SV4D \cite{xie2024sv4d, yao2025sv4d}. WAN $2.1$ is a powerful video foundation model based on the diffusion transformer framework. It uses a spatio-temporal variational encoder (VAE) to capture both spatial and temporal aspects of videos and is trained on a large-scale dataset of billions of images and videos. WAN $2.1$ is available in two model sizes: $1.3B$ and $14B$ parameters, targeting efficiency and performance, respectively. We use the $14B$ variant for our experiments. All our results for image to video generation are generated using the HuggingFace demo, which offers a distilled version of WAN $2.1$ optimized for fast inference in just $4$ steps using CausVid LoRA. SV4D \cite{xie2024sv4d, yao2025sv4d} on the other hand is a latent video diffusion model designed for generating {\em multi-view\/} and {\em multi-frame\/} consistent dynamic 3D content from a single-view input video which enables efficient 4D asset optimization. SV4D is a {\em generalizable\/} model trained on a {\em large corpus of dynamic scenes\/} from Objaverse \cite{deitke2023objaverse} unlike ours which is trained on only {\em few-shot\/} reference motion samples. 

For baseline comparisons for multi-view motion generation, we use WAN $2.1$ to generate a video from an image using a text prompt and then apply SV4D to convert the video into multi-view sequences. We denote this configuration of the baseline as WAN2.1+SV4D.

As text prompt is not a robust way to control the part motion as observed in our experiments, we create another configuration where a generalizable I2V model like PuppetMaster \cite{li2025puppet} which is trained with more explicit prompt control like ``drag" is used. Note that, these drags are manually annotated for a large collection of dynamic content from Objaverse. Once trained, this model can synthesize a video depicting part-level motion faithful to the given drag interactions. We combine such a I2V diffusion model which has more fine-grained control on part motion with SV4D to create multi-view videos. We denote this baseline configuration in our experiments as PM+SV4D.
\subsubsection{3D Motion Axis Parameter Estimation Baselines.} Our pipeline estimates {\em 3D motion attribute\/} parameters from a static, segmented 3D mesh using motion outputs from a controllable multi-view motion diffusion model. To compare our 3D joint estimation results we benchmark against two baselines Shape2Motion (S2M) \cite{wang2019shape2motion} and Openable Part Detection (OPD) \cite{jiang2022opd}. Shape2Motion predicts motion parameters from a point cloud and is trained end-to-end with 3D ground truth motion axis parameters. OPD, on the other hand, estimates motion parameters from a single image using an object detector backbone that predicts segmentation masks, motion type, and motion parameters. We compare with against both these baselines in a few-shot setting by retraining them with our train and test split.
% \input{figures/mask_effect}
\subsection{Results Discussions.} 
\subsubsection{3D Motion Axis Estimation Results.} As shown in Table \ref{tab: partnet_sapian_quant} \& \ref{tab:motion_parameter_estimation_gen}, and Fig. \ref{fig:results_acd} \& \ref{fig:results_ps}, our method predicts plausible motion parameters without using 3D annotations, beating the prior state-of-the-art methods by a large margin, especially in angular error metrics (\texttt{MAE}). Shape2Motion on the other hand, outperforms OPD (Table \ref{tab: partnet_sapian_quant}) since it leverages point clouds (explicit 3D representation) and is trained in 3D-domain making the optimization task relatively easier, whereas, OPD relies on {\em single-image\/} inputs which makes the overall optimization task of making predictions in 3D from only images relatively challenging. In {\em zero-shot \/} generalization experiment, Shape2Motion struggles to show good generalization (Table \ref{tab:motion_parameter_estimation_gen}) due to limited generalization capability of the 3D backbone network in a few-shot setting. In contrast, our method generalizes well, showcasing the effectiveness of the diffusion prior in learning part dynamics and the 3D motion axis parameter estimation step which reliably lifts the motion from 2D to 3D space. Additionally, our algorithmic optimization strategy simplifies the motion axis estimation step by transforming it from a continuous regression task into a discrete classification task. This reformulation allows us to search for the optimal solution within a fixed solution space, making the optimization process more tractable compared to the regression-based approaches used in prior works. As a result, we are able to achieve more accurate outcomes for 3D motion axis parameter estimation.
\input{figures/qualitative_3d_ps}
\subsubsection{Multi-view Motion Generation Results.} Beyond 3D motion parameter estimation, we also compare our multi-view motion generation results with the proposed baselines on diverse categories of objects from PartNet-Mobility \cite{mo2019partnet} and Objaverse \cite{deitke2023objaverse} datasets like {\em trashcan, dishwasher, display, lamp and stapler\/}. Fig.~\ref{fig:results_mv} presents the comparative video outputs from the I2V diffusion models. Because ours is a single-stage pipeline where we directly predict multi-view motion outputs, we directly compare the multi-view outputs of our method with the baselines and skip I2V comparison. As shown in the Fig. ~\ref{fig:results_mv} (left), despite WAN2.1 being a large model trained on a large-scale dataset, it lacks a clear understanding of part-specific dynamics. This results into incorrect outputs in several cases when motion is controlled using only a text prompt. For example, for the {\em lamp\/} and {\em display\/} categories, the model generates videos where the entire lamp rotates upside down instead of just the lamp head. In the case of the {\em dishwasher\/}, the model fails to understand how the door opens based on the input and instead produces a motion pattern it may have encountered during training. Additionally, models with more explicit control, such as Puppetmaster, often struggle to disambiguate between parts using only drag prompts, leading to incorrect motion and poor quality video for SV4D. Fig. ~\ref{fig:results_sv4d} and Table ~\ref{tab:video_generation_comparison} shows the qualitative and quantitative comparison results respectively of our multi-view motion output with the proposed baselines. Videos from each view is colored differently in Fig. ~\ref{fig:results_sv4d} where two different colors indicate two different views. We only show two views for simplicity, however, in actual implementation we generate $4$ views. As can be seen in Fig. ~\ref{fig:results_sv4d} and Table ~\ref{tab:video_generation_comparison} our method outperforms the baselines in terms of both qualitative and quantitative results. Not only the output of the baselines is affected by the output from I2V diffusion model, but also the final multi-view consistency of the motion can be affected by the geometric inconsistencies introduced by SV4D, leading to error propagation in this two-stage pipeline. This can be especially observed in the output of trashcan and dishwasher where SV4D is not able to faithfully reconstruct the dynamic content in its multi-view motion output. In regards to video quality metrics, Table \ref{tab:video_generation_comparison} show that our method achieves best $\texttt{CLIP}$, $\texttt{PSNR}$, $\texttt{LPIPS}$ and $\texttt{FVD}$ scores which shows that our method is able to generate 3D consistent output in a controllable manner along with successful articulation (Table ~\ref{tab: partnet_sapian_quant} \& ~\ref{tab:motion_parameter_estimation_gen}). More results on variety of test shapes from ACD \cite{iliash2024s2o}, Objaverse \cite{deitke2023objaverse, deitke2024objaverse} and PartNet-Mobility are shown in Fig. ~\ref{fig:acd_new_1}, ~\ref{fig:acd_new_2}, ~\ref{fig:objaverse_new_3}, ~\ref{fig:ps_new_4} respectively.
\input{tables/mv_results}
\input{figures/mask_effect}
\section{Ablations} 
We perform various ablations of our method to show the effectiveness of each component in our pipeline. First, we perform an ablation on how our algorithm based optimization yields more plausible solution compared directly optimizing the points in the rest state using chamfer distance loss. Table ~\ref{tab:dir_vs_algo.} and Fig. ~\ref{fig:dir_vs_algo} shows the quantitative and qualitative results of direct vs algorithmic optimization. As can be seen in Fig. ~\ref{fig:dir_vs_algo}, optimizing the lamp head directly with chamfer distance loss yields incorrect output because of noisy point cloud initialization obtained after reconstruction. Because we reformulate a continuous regression-based task of motion axis estimation into a discrete classification task, it makes the optimization process more tractable; hence, we are able to achieve more accurate outcome as seen in the Fig. ~\ref{fig:dir_vs_algo}. In Table \ref{tab:num_vids} we show how the generation quality of multi-view videos is affected as we increase the number of videos for finetuning. As can be seen in Table \ref{tab:num_vids} multi-view and temporal consistency significantly drop as we reduce the number of training videos, which is reflected in the metrics, especially in \texttt{PSNR} which evaluates pixel-level correspondences between the generated output and ground truth. In support to this, in Fig. ~\ref{fig:num_videos} we show the effect of using the guidance of the diffusion model trained with increasing number of videos in final motion axis estimation. As can be seen, increasing the number of videos for training yields better geometrically consistent videos which in general yields better reconstruction of articulated point cloud, which helps in better estimation of the motion axis. Finally, in Fig. \ref{fig:mask_effect} we show the motion controllability of our method. As can be seen, by providing the appropriate part mask as prompt, we can control the spatial location of part motion for same object. The spatial controllability of motion plays a key role in enabling the articulation of different parts of the same object. By simply modifying the mask used as a prompt, we can generate appropriate motion for the desired part of the shape. This is illustrated in Fig.~\ref{fig:multi-part}, where we present multi-part 3D articulation results across various 3D shapes. In each case, we adjust the prompt location based on the specific part to be articulated and then optimize the 3D motion parameters using guidance from the generated multi-view motion output. Multiple inference runs are performed by changing the mask location to produce distinct part-specific motions. Finally, in Fig.~\ref{fig:training_samples}, we present the training samples used during the finetuning of our diffusion model for one of the category from PartNet-Mobility dataset (StorageFurniture), along with the test shapes from the ACD dataset. As shown in the figure, there are substantial structural differences between the training and test objects, highlighting the strong generalization ability of our method.

\input{figures/dir_vs_heu}
\input{figures/abl_num_vids}
 \input{figures/multi_part}
% \input{tables/ablations}



==> remove/7_revisions.tex <==
\section{Cover Letter}
\label{sec:revision}

\noindent Dear Associate Editor and Reviewers,

\vspace{3mm}

\noindent We sincerely thank you for the thorough evaluation of our manuscript and for the constructive feedback provided during the review process. We greatly appreciate the time and effort invested in assessing our work.

In this revision, we have carefully addressed all the concerns and suggestions raised by the reviewers. Below, we provide a structured summary of the revisions for each point raised by the reviewer. For clarity, we organize the responses into two categories: (1) weaknesses identified by the reviewers and (2) suggestions for improvement. For each point, we provide a response and indicate the corresponding sections in the revised manuscript where changes have been made.

We hope that the revisions and clarifications satisfactorily address the reviewers’ concerns and improve the overall quality and clarity of the paper.

Sincerely, 
The Authors

\subsection{Weaknesses}

\begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=2pt, leftmargin=*]
\item {\em The method assumes the input mesh is already segmented or relies on off-the-shelf segmenters. If the segmentation is ambiguous (which is common in raw Objaverse data), the motion mask control will fail. The paper briefly mentions this but could elaborate on failure cases caused by poor segmentation.} 

\noindent \textbf{Answer.} \rev{We perform an ablation to show the effect on motion generation with erroneous masks predictions from foundation models like \cite{ravi2024sam2segmentimages}. The results are discussed in Sec. \ref{sec:ablations} and are highlighted. We show that robustness to segmentation quality can be improved by small data augmentation during finetuning step.}

\item {\em The current framework assumes a binary segmentation: a moving part against a static rest-state background. This formulation inherently fails to model coupled or hierarchical motion, where the movement of a child part depends on the parent part (e.g., a handle moving with a door, or a laptop screen moving relative to a base that might itself be moving). Running separate inference steps is insufficient because the second step would treat the parent part as static, breaking the relative mechanical linkage.}

\noindent \textbf{Answer.} \rev{Currently, our method only supports \textit{multiple part motion} against the static frame and cannot represent coupled or hierarchical motion. We discussion this in Sec. \ref{sec:limitations}. }

\item {\em The paper claims strong generalization capabilities under a "few-shot setting" , where the model is finetuned on a small collection of reference motion frames. However, the boundary of this generalization is ambiguous. It is unclear whether the model learns the underlying physics of articulation types (e.g., the concept of a hinge) or merely memorizes specific 2D pixel-flow trajectories associated with mask locations from the training set (e.g., "pixels in the mask move left"). If the test set contains a motion type structurally distinct from the few-shot training examples (e.g., a vertical folding garage door vs. a standard swinging door), it would be interesting to see how the model performs in such out-of-distribution scenarios.
}

\noindent\textbf{Answer.} \rev{Currently, our method requires atleast one video sample for the model to learn all the motion dynamics. }

\end{enumerate}

\subsection{Suggestions}
\begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=2pt, leftmargin=*]

\item {\em If the proposed method is capable of handling kinematic chains, the authors are strongly encouraged to include a demonstration or explanation of this mechanism in the revision. Conversely, if the current pipeline treats parts independently against a static background, it would be beneficial to explicitly discuss this distinction between "independent multi-part motion" and "hierarchical motion" in the limitations section to clarify the method's scope.
}

\noindent \textbf{Answer.} \rev{Thank you for pointing this out. At present, our model supports only independent multi-part motion. We discuss this limitation in Sec. \ref{sec:limitations}.}

\item  {\em The authors can clarify the diversity of motion types present in the few-shot training set versus the test set. The revision should distinguish between "geometric generalization" (applying known motions to new shapes) and "kinematic generalization" (inferring new motion types). If the method cannot generalize to motion types (e.g., trajectories) unseen during the few-shot fine tuning, this should be clearly stated as a limitation. A discussion on "Out-of-Distribution" motion types would significantly strengthen the technical rigor.}

\noindent \textbf{Answer.} \rev{We would like to clarify that currently our model does not generalize to different kinematic variations and this direction is left for future exploration. We highlight and discuss this specific limitation in Sec. \ref{sec:limitations}.}

% We note that kinematic generalization, i.e., inferring new motion types, requires extrapolating motion dynamics beyond the support of the few-shot fine-tuning data. Achieving this would require learning additional priors or “rules,” such as explicit joint concepts, physical constraints, or motion-centric representations. In contrast, the proposed method is designed to support geometric generalization, i.e., applying known motion patterns observed during few-shot fine-tuning to new shapes with significant structural variations. Fig. \ref{fig:training_samples} provides examples of the types of structural variations our model can handle. This design choice is motivated by the limited availability of articulated motion datasets and the strong ability of diffusion models to represent object geometry. By learning a motion pattern under limited supervision, the model can effectively transfer this pattern to novel shapes with diverse structures. We have highlighted this in the limitations section in the revised manuscript.

\item {\em To fully validate the advantage of the proposed piecewise rigid constraint, it would be persuasive to include a comparison against general-purpose mesh animation algorithms (e.g., AnimateAnyMesh or similar generic 4D approaches). Explicitly contrasting ATOP with methods that typically rely on soft deformations would highlight its superior ability to preserve structural integrity and avoid the non-rigid distortions often seen in general baselines.
}

\noindent\textbf{Answer.} \rev{Thank you for highlighting this insightful point. We have added a qualitative comparison and discussion between our method and approaches based on soft deformations, such as AnimateAnyMesh \cite{wu2025animateanymesh}. The discussion is included in Sec. \ref{experiments} and the comparison figure is shown in Fig. \ref{fig:rigid_vs_soft}.}

\end{enumerate}


==> remove/ab_rebut.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt} % Slightly adjust column spacing for balance
\renewcommand{\arraystretch}{1.1} % Adjust row spacing for readability
\footnotesize % Use a smaller font for compactness
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Method} & \textbf{CLIP} $(\uparrow)$ & \textbf{FVD} $(\downarrow)$ & \textbf{LPIPS} $(\downarrow)$ & \textbf{PSNR} $(\uparrow)$ \\
\midrule
ST-Attn & 24.71 & 887.3 & 0.131 & 22.13 \\
All-vs-First & 23.57 & 922.6 & 0.139 & 21.27 \\
\bottomrule
\end{tabular}
\vspace{-5pt} % Reduce space below the table
\caption{Full ST-Attn vs One-to-all Attention.}
\label{tab:full_vs_one}
\end{table}


==> remove/ablations.tex <==
% \begin{table}[!htb]
% \vspace{-0.2in}
%     % \caption{Global caption}
%     \begin{minipage}{.5\linewidth}
%           \centering
%         \caption{\textbf{Ablation} Opt. vs. Algo.}
%         \label{tab:runtime}
%         \vspace{-0.1in}
%         \small
%         \begin{tabular}{c|cc}
% \hline
% Methods       & Ag Er $\downarrow$          & Ps Er$\downarrow$                   \\ \hline
% % B-I   & 1133         & 3.00 hr          \\
% Dir. Opt.        & 1.57          & 0.11           \\
% \cellcolor{blue!15} Algo. Opt. & \cellcolor{blue!15}\textbf{0.98} & \cellcolor{blue!15}\bf 0.07 \\ \hline
% \end{tabular}
% \label{tab:dir_vs_algo.}
%     \end{minipage}%
%     \begin{minipage}{.5\linewidth}
%  \caption{\textbf{Ablation} on \# videos}
%  \label{tab:user}
%       \vspace{-0.1in}
%       \footnotesize
%       \centering
% \begin{tabular}{c|cc}
% \hline
% \# Vids & FVD $\downarrow$ & PSNR $\uparrow$ \\ \hline
% % B-I     & 3.14                 \\
% 1    & 1296.2            &  14.23     \\
% 4  & 1172.3             & 17.78   \\ \hline

% \cellcolor{blue!15}  8   & \cellcolor{blue!15}\bf 983.7 & \cellcolor{blue!15}\bf{19.83}                \\ \hline
% \end{tabular}
% \label{tab:num_vids}
%     \end{minipage}
%     % \vspace{-0.15in}
% \end{table}



==> remove/lamp_rebut.tex <==
\begin{figure}[!t]
\vspace{-0.15in}
\centering
   \includegraphics[scale=0.5]{images/rebut_fig.png}
   \vspace{-0.12in}
    \caption{Motion variation using different text prompts}

\label{fig:lamp_art}
\end{figure}

==> remove/motion_parameter_generalization_results.tex <==
\begin{table*}[t!]
% \small
\centering
\begin{tabular}{c|c|cccccccc|c}
\hline
\multirow{2}{*}{\textbf{Metric}}                            & \multirow{2}{*}{\textbf{Method}} & \multicolumn{9}{c}{\textbf{Categories}}                                                     \\ \cline{3-11} 
                                                   &                         & Armoire & Cabinet & NightStand & Table & Microwave & Oven & Refrigerator & Washer & Mean \\ \hline
\multirow{3}{*}{Ang Err $\downarrow$}& S2M                     &      17.32   &    19.34     &       22.37     &    21.62   &    23.56       &  22.56    &    25.42    &   19.77     &    21.49  \\
                                                   & OPD                     &     12.37    &    9.26     &     10.62       &   8.43    &     16.46      &   14.93   &   13.62     &   11.21     &   12.11   \\
                                                   & Ours                    &  \cellcolor{blue!15} \textbf{2.83}      &    \cellcolor{blue!15}\textbf{3.29}     &     \cellcolor{blue!15}\textbf{3.92}       &   \cellcolor{blue!15}\textbf{2.39}    &     \cellcolor{blue!15}\textbf{3.52}      &    \cellcolor{blue!15}\textbf{3.34}  &  \cellcolor{blue!15}\textbf{2.96}      &    \cellcolor{blue!15}\textbf{6.75}    &  \cellcolor{blue!15}\textbf{3.63}    \\ \hline
\multirow{3}{*}{Pos Err $\downarrow$} & S2M                     &    0.15     &    0.22     &      \cellcolor{blue!15}  \textbf{0.19}    & \cellcolor{blue!15} \textbf{0.16}     &      0.16     &   0.13   &   0.15    &    0.15    &   0.17   \\
                                                   & OPD                     &    0.22     &     0.25    &   0.19         &   0.21    &     0.25      &   0.27   &   0.19     &   0.18     &  0.22    \\
                                                & Ours                    &  \cellcolor{blue!15} \textbf{0.06}      & \cellcolor{blue!15}  \textbf{0.07}      &     0.54       &   0.19    & \cellcolor{blue!15} \textbf{0.12}         &   \cellcolor{blue!15}\textbf{0.09}   &     \cellcolor{blue!15}\textbf{0.11}   &    \cellcolor{blue!15}\textbf{0.04}    &   \cellcolor{blue!15}\textbf{0.16}   \\ \hline
\end{tabular}
\vspace{2mm}
\caption{
Quantitative evaluation of zero-shot generalization on ACD dataset \cite{iliash2024s2o} curated by \cite{liu2024singapo}. Motion parameters are optimized with guidance personalized motion diffusion model with {\em no new finetuning \/}.
}
\label{tab:motion_parameter_estimation_gen}
\end{table*}


==> remove/pipeline_cross_attention.tex <==

\begin{figure}
    \includegraphics[height=6cm]{images/cross_attention_pipeline.png}

\caption{
    Cross Attention Block
}
\label{fig:pipeline-ca}
\end{figure}

==> remove/pipeline_overview.tex <==
\begin{figure*}
\vspace{-1em}
    \includegraphics[width=\textwidth]{images/pipeline_v3.png}
\caption{Pipeline Overview: Given a small collection of multi-view videos belonging to the same category our goal is to learn a category specific part motion by finetuning a multi-view image diffusion model. For this, noisy latents of the multi-view videos are denoised using the UNet blocks. Appearance information is injected into the UNet through conditioning, and controllability in part motion is achieved by injecting part masks into the diffusion process. Once finetuned, we can adapt the model for a new mesh and optimize the motion axis parameters with score distillation loss using the guidance of the diffusion model.
\sn{This figure should focus more on standalone Single-Image to MV-Video Generation pipeline with details of internal blocks like affine transformation clubbed into one or separate like now.}
}
\label{fig:pipeline}
\vspace{-1.5em}
\end{figure*}

==> remove/results_acd.tex <==
\begin{figure*}
    \includegraphics[width=\textwidth]{images/result_2.png}

\caption{Qualititative results of generalization of Multi-view video generation and 3D Motion Axis prediction on ACD dataset \cite{iliash2024s2o}.}
\label{fig:acd_1}
\end{figure*}


\begin{figure*}
    \includegraphics[width=\textwidth]{images/result_3.png}

\caption{Qualititative results of generalization of Multi-view video generation and 3D Motion Axis prediction on ACD dataset \cite{iliash2024s2o}.}
\label{fig:acd_2}
\end{figure*}


==> remove/results_ps.tex <==
\begin{figure*}
    \includegraphics[height=\textheight]{images/result_1.png}

\caption{Qualititative results of Multi-View Video Generation and 3D motion axis prediction on PartNet Sapian Dataset.}
\label{fig:results partnet sapian}
\end{figure*}



==> remove/t2i_articulation.tex <==
% \begin{figure}
%    \includegraphics[scale=1.25]
%    {images/sd_articulation.png}
%     \caption{Samples generated from a Text to Image diffusion model \cite{stable_diffusion}. As can be seen, unlike video diffusion model (Fig. \ref{fig:diff_articulation}) image diffusion models have relatively higher articulation awareness which eases the finetuning process.}
% \label{fig:t2i_articulation}
% \vspace{-5mm}
% \end{figure}

==> remove/teaser.tex <==



% \begin{figure*}[t!]
%   \includegraphics[width=0.9\linewith]{images/teaser_v2.png}
%   \centering
%   \caption{Given a textured mesh in rest state (left), the part to articulate (highlighted), and a text prompt as input, we first generate multi-view videos (middle) of plausible part articulation using our personalized diffusion model. We then transfer the motion from the generated videos back to the 3D mesh (right). The input meshes are the {\em top retrieval results\/} from Objaverse \cite{deitke2024objaverse} for ``Trash can" and ``Lamp."}
%   \label{fig:teaser}
% \end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/teaser_v2.png}
    \caption{Given a textured mesh in rest state (left), the part to articulate (highlighted), and a text prompt as input, we first generate multi-view videos (middle) of plausible part articulation using our personalized diffusion model. We then transfer the motion from the generated videos back to the 3D mesh (right). The input meshes are the {\em top retrieval results\/} from Objaverse \cite{deitke2024objaverse} for ``Trash can" and ``Lamp."}
    \label{fig:teaser}
\end{figure*}

